Wooly Graphs : A Mathematical Framework For Knitting

This paper aims to develop a mathematical foundation to model knitting with graphs. We provide a precise definition for knit objects with a knot theoretic component and propose a simple undirected graph, a simple directed graph, and a directed multigraph model for any arbitrary knit object. Using these models, we propose natural categories related to the complexity of knitting structures. We use these categories to explore the hardness of determining whether a knit object of each class exists for a given graph. We show that while this problem is NP-hard in general, under specific cases, there are linear and polynomial time algorithms which take advantage of unique properties of common knitting techniques. This work aims to bridge the gap between textile arts and graph theory, offering a useful and rigorous framework for analyzing knitting objects using their corresponding graphs and for generating knitting objects from graphs.

==> sections/04-results.tex <==
\section{Main Results}
% file for main results which we must select a subset of to present in full. 

\subsection{Problem 1}
\begin{problem}
    \problemtitle{Problem 1}
    \probleminput{An abstract directed acyclic graph}
    \problemquestion{Find a Hamiltonian path (to model the yarn course) under the constraint of having only the \emph{allowed configurations} connecting the nodes as the remaining edges not being part of the path.}
\end{problem}

\BB{Note we must also exclude using two yarns in 1 stitch, or alternately having two stitches occupying the same node -- this would allow a stitch to be on the hamiltonian paths of two yarns -- `simple' knitting must exclude this.}

\begin{table}[htb]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    Indeg  & 0 & 1 & 2 & $\geq 3$ \\
    \hline
    Outdeg & & & &  \\
    \hline
    0 & non-feasible & non-feasible & must be  & non-feasible \\
     &  & & a source &  \\
    \hline
    1 & non-feasible & non-feasible & cannot be & must be a sink \\
     & &  & a source &  \\
    \hline
    2 & must be  & cannot be  & can be all & intermediate \\
    & a source &  a sink &  &  intermediate \\
    \hline
    $\geq 3$ & non-feasible & must be  & must be  & non-feasible \\
    & & a source & intermediate & \\
    \hline
    \end{tabular}
    \caption{Combinations of in- and outdegrees and their implications on feasibility.}
    \label{tab:degrees-overview}
\end{table}
\BB{Details for Problem 1: 
Restriction provides a covering. We will identify potential sources (linear time) and begin at an arbitrary source. Now, we need to partition edges into two types: hamiltonian (blue) and stitching (red). Now in the sense of a mincostflow, we will double each of our vertices to separate incoming and outgoing edges, joining the duplicated vertices by a single edge from in to out. We will assign a minimum flow of 1 to each of these new edges. Now, we must cover all edges of our dag with paths from sources to sinks. We will accomplish this by starting from an arbitrary vertex and following an un-marked edge if possible at each consecutive vertex reached until either we reach a sink OR we reach a vertex with only marked outgoing edges -- in the latter case, we pick the index of one of the outgoing edges of this final vertex and mark all edges in this path with that index. Repeat until all edges are marked. This will take linear time. Now we need to merge paths to eliminate redundant connections for the mincostflow, here we will use the restriction against many-to-many vertices to prevent branching decisions. Now starting from a sink, we look at the incoming paths which must be adjacent -- we will mark all edges not connected to a source or sink which connect these two paths as on the hamiltonian path -- this induces a cheaper flow. Since we do not have many-many vertices, we need }

For problem 1, we think that a MinCostFlow model can be used. Given the restrictions on the nodes based on their degree (see Table~\ref{tab:degrees-overview}, we can enforce both a covering as well as the restrictions from the loop intersections (red edges). To be shown: Every solution is feasible for knitting and if there is a knittable solution the flow problem has a solution.


\begin{problem}
    \problemtitle{Problem 1.1 Plane Directed Multipath Cover}
    \probleminput{Plane directed Graph}
    \problemquestion{Find $k$ paths (non-intersecting - vertex disjoint) that cover the full graph. What about fairness - how much can be covered with each path, balanced way? 
    \BB{Do the $k$ covers for minimum $k$ partition the graph into sub-graphs on which the length of each cover is already maximal?} At most two outgoing OR incoming edges (otherwise we have a forbidden configuration with at least two incoming AND outgoing edges)}
\end{problem}

\begin{problem}
    \problemtitle{Problem 1.3 Simple Embedding}
    \probleminput{An abstract directed acyclic knittable graph, with correct blue/red coloring for knitting}
    \problemquestion{Decide if the input has a simple embedding, and calculate it.}
    \BB{I believe that this is a twist measurement process -- follow the Hamiltonian path -- this induces an ordering of stitches AND the stitches below them. We can check if we ever swap this ordering (a cable stitch or a twist and sew together, etc...) Count the number of times stitches swap in the order, this measures the genus of the embedding. If the genus turns out to be 1, then the object has a simple embedding AND the ordering of the stitches induces the embedding.}
\end{problem}

\begin{theorem}
    \label{thm:test-simplicity}
    Given a 1-knittable directed graph $G$ with edge coloring $c$, it can be decided whether $G$ is simply knittable and if, a corresponding plane embedding $\Gamma$ of $G$ can be computed in polynomial time. \BB{See above, I believe that this is linear time by counting stitch order changes}
\end{theorem}

\begin{proof}
    
\end{proof}


Similar to bimodality testing: Split every vertex into a four-cycle, where every vertex becomes one badge of edges, and test if the resulting graph is bimodal.

\subsection{Problem 2: Recognizing simple knittable non-colored graphs}

\begin{problem}
    \problemtitle{Problem 2}
    \probleminput{A plane undirected graph}
    \problemquestion{Direct the graph and color the edges blue or red such that the graph is knittable, i.e.\ the blue edges form a path that is Hamiltonian and the red edges are allowed configurations.}
\end{problem}

If we allow "all" red configurations, then we still cannot freely assign edges to adhere to the restrictions as local decisions on the direction of red edges might be inconsistent. Our assumption is that the problem is hard. \BB{computing a Hamiltonian path on an undirected simple graph $\longleftrightarrow$ knittability, also determines the coloring of the graph up to the red edge directions. Red edge directions can be determined by the hamiltonian path ordering where they must always point from lower Hamiltonian index to higher.}

3-regular planar graph reduction - just choose a single edge (iterate through all), delete it and use our approach to find a path. If existing, this creates a cycle in the original since every path in our algorithm has to start and end at a degree 2 vertex. Also every Hamiltonian path starting and ending in the degree 2 vertices will leave a red matching, so the conditions are always fulfilled.

\begin{problem}
    \problemtitle{Problem 2.2}
    \probleminput{A plane undirected internally four-connected graph}
    \problemquestion{Direct the graph and color the edges blue or red such that the graph is knittable, i.e.\ the blue edges form a path/several paths that is Hamiltonian and the red edges are allowed configurations. } \BB{Some notes: Tutte's theorem guarantees such graphs will have a hamiltonian path. Internally 4-connected graphs will have at least 2 orientation choices for the hamiltonian path and finding either of them will do, this amounts to only using the plane to orient each stitch and testing whether By making a path partition and then coloring edges red or blue while merging paths, this can be accomplished in linear time \cite{chiba1989hamiltonian}.}
\end{problem}

\subsection{Problem: Characterization of graphs knittable with arbitrary many threads}

\begin{problem}
    \problemtitle{Problem 3}
    \probleminput{A graph that is uncolored and or undirected}
    \problemquestion{Is there some $k$ such that the graph is (simply) $k$-knittable?}
\end{problem}
\BB{This is just the k-path cover problem which is np-hard}

\begin{problem}
    \problemtitle{Problem 4}
    \probleminput{A directed multigraph}
    \problemquestion{Can this be a yarn graph for a $k$-knittable object?}
\end{problem}
\BB{
Linear time, check for odd order vertices -- these are the sources and sinks. If the extra vertex is outgoing it is a source and vice versa. $k$ can be measured by starting at sources and following the edges of each vertex and coming back whenever possible, marking the remaining outgoing edge as on the path. Continue until no vertices are left un-touched. Now in linear time, count the disjoint paths, this is the minimum $k$. 
}

\subsection{Cable-width}

Motivation: Knitted Pieces are generally not planar!

\begin{figure}[!htb]
    \centering
    \includegraphics[width=.35\textwidth]{Figures/cable-pattern.pdf}
    \caption{Graph of a cable knitting pattern}
    \label{fig:cable-pattern}
\end{figure}

\begin{definition}[cable width]
    Let $G$ be a graph and $\Gamma$ be a (not necessarily planar) drawing of $G$. The \emph{cable width} of $G$ is the minimal number $k$, such that $G$ can be drawn such blue edges pairwise do not cross, every vertex has a regular edge system, and the edge-size of the biggest component crossing-graph is $k$.
\end{definition}



==> sections/defining_knitting.tex <==
First, we must discuss how we are defining knitting and knitting graphs within the context of this paper. 

We will start with the simplest form of knitting.

\begin{definition}[$1$-Knit Object]
    A \emph{$1$-knit object} $O$ is an arrangement of interlocking loops in a single piece of yarn such that connecting the two ends of the piece of yarn creates the un-knot. Furthermore at least one loop must be secured only by another loop passing through it.  
\end{definition}

This definition gives us the structure of knitting, loops or stitches, as seen in Fig:~\ref{fig:basic-knitting-single-stitch}. This figure shows a single row, in red, to show the path of the yarn.  In addition, we ensure that the knit object is not trivial by including that we must have one loop secured only by another loop. 

Now we will extend this definition by allowing more than one yarn. In knitting, techniques using more than one yarn are common, including fair isle, stripes, double knitting, intarsia, and other colorwork.

\begin{definition}[$k$-Knit Object]
    A \emph{$k$-knit object} $O$ is a collection of $k$ yarns arranged into loops which interlock and for which each independent yarn, joined end-to-end forms the un-knot. Furthermore at least one loop must be secured only by another loop passing through it. 
\end{definition}

From here, we will define a knitting graph. We will start by 

\begin{definition}[Knitting Vertices]
    A \emph{knitting vertex} $v$ is one loop of yarn which is either closed or held by another stitch passing through it. 
\end{definition}

\begin{figure}[ht]
\includegraphics[width=0.4\textwidth]{Figures/single_stitch.png}
\caption{An example of a graph on stockinette stitch knitting.  We highlight the Hamiltonian path in red and the extra edges for the Eulerian path in blue.  This is a subsection of knitting and the graph would extend to all stitches in general.}
\end{figure}\label{basic-knitting-single-stitch}

\begin{definition}[Knitting Graph]
    A \emph{knitting graph} $G = (V, E)$ for a knit object $O$ is a simple graph consisting of all knitting vertices $V$ and edges $E$ connecting each vertex to any other vertex that: (1) is sequential along the yarn with this stitch, (2) is passed through by this stitch, or (3) passes through this stitch. 
\end{definition}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/ham_eul_example.png}
    \caption{An example of the Eulerian knitted graph.  Here, the edges that are on the Hamiltonian are shown in black and the ones only on the Eulerian are shown in blue}
    \label{fig:eulerian_example}
\end{figure}

\begin{definition}[Yarn Graph]
The {yarn graph} $Y = (V, E)$ for a knit object $O$ is a  directed multi-graph consisting of all knitting vertices $V$ for the object and edges with edges $E$ for the path of the yarn as it passes through stitches.
\end{definition}

\textbf{Note:} The knitting graph is an un-directed subset of the yarn graph.
